Hierarchical Grammar-Induced Geometry for Data-Efficient Molecular Property Prediction

The prediction of molecular properties is a crucial task in the field of material and drug discovery. The potential benefits of using deep learning techniques are reflected in the wealth of recent literature. Still, these techniques are faced with a common challenge in practice: Labeled data are limited by the cost of manual extraction from literature and laborious experimentation. In this work, we propose a data-efficient property predictor by utilizing a learnable hierarchical molecular grammar that can generate molecules from grammar production rules. Such a grammar induces an explicit geometry of the space of molecular graphs, which provides an informative prior on molecular structural similarity. The property prediction is performed using graph neural diffusion over the grammar-induced geometry. On both small and large datasets, our evaluation shows that this approach outperforms a wide spectrum of baselines, including supervised and pre-trained graph neural networks. We include a detailed ablation study and further analysis of our solution, showing its effectiveness in cases with extremely limited data. Code is available at https://github.com/gmh14/Geo-DEG.

==> sections/approach.tex <==
\section{Grammar-induced intrinsic geometry for property prediction}
\label{sec:approach}
% \mh{Consider to remove this section if too much overlap with the intro}

\textbf{Overall Pipeline, Figure~\ref{fig:motivation}.} \mh{step bullet points}
% \mh{need to polish since it overlaps with intro}
% \mh{Need to correct a lot of mistakes}
% \mh{dont mention anything related to generative model in the method section since we dont contain thorough experiments on molecular generation. Treat the joint optimization of generative model and property predictor as a byproduct of the system, but not the major goal.}
% Our goal is to design a grammar-based, geometric \pd{geometric property is wrong here}property predictor for molecules that can be applied in a grammar-based generation system.
% \footnote{We focus on a grammar-based molecule generation scenario, where the goal is to predict properties for the molecules generated by the grammar, but the approach can be applied for property prediction over arbitrary molecules (see our experiments), then the latter are given as additional input to the grammar learning.} 
Our goal is to design a molecular property predictor based on the grammar-induced geometry. 
More specifically, given a set of molecules, we learn a geometry for the space of molecules in the form of a graph, where each molecule, as well as each \st{intermediate graph} \textcolor{magenta}{partial molecule}, is represented as a node of the \st{geometry} \textcolor{magenta}{graph}.
A key characteristic of this geometry is that structurally similar molecules are closer in distance along the geometry.
Property prediction is achieved using a graph diffusion model over the geometry.
To this end, we propose a \emph{hierarchical molecular grammar} consisting of two graph grammars: a predefined \emph{meta grammar} with well-characterized attributes that can generate all tree structures in a complete yet compact manner, and a learnable \emph{molecular grammar} which can convert the trees generated by the meta grammar into molecular graphs.
The geometry is determined by a grammar DAG which represents all the \st{intermediate graphs} \textcolor{magenta}{(partial) molecules} and the production sequences enumerated by the hierarchical molecular grammar.
While being of combinatorial complexity, the part of the grammar DAG related to the meta grammar can be constructed offline and generalized to all molecular datasets, thus reducing the computational cost.
We then perform graph diffusion on this explicit grammar-induced geometry to predict property values, and jointly optimize both the induced geometry and the graph diffusion model.
% More specifically, we learn an \emph{intrinsic geometry over molecules, in form of a graph structure}, %containing molecules both within and outside of the training data, 
% along with a {graph diffusion model} that is applied over that graph and predicts the properties of newly generated molecules.
% To this end, we propose \emph{hierarchical molecular grammars}, graph grammars as introduced in Section~\ref{sec:preliminaries} but of a specific shape that allows to split the grammar into a constant, data-independent part and one that is learned at runtime. 
% Our approach centers around molecules as junction trees; consider the tree nodes as nonterminal nodes, each expandable into a subgraph. Based on this idea, we consider \emph{meta rules} that generate the tree structures of the junction trees using only nonterminal nodes, and \emph{molecular rules}, which generate molecule fragments and hence expand the trees into molecules.
% % We show that these restrictions do not decrease expressivity.
% %
% As outlined in Figure~\ref{fig:metagrammarJT},
% our geometry is then based on (1) a \emph{meta DAG} constructed offline based on % given 
% meta rules  and (2) molecular graphs that are attached as leaves to the leaves of the meta DAG. Observe that each node in the meta DAG represents a set of potential junction trees (i.e., with same first tree component).
% At runtime, the input consists of a set of molecules together with their property values.
% %In order to learn 
% To complete the geometry, we then learn molecular rules accompanying the meta rules, which provide possibilities for how a molecule can be split into a junction tree. The latter determine where the molecule is attached to the meta DAG in that we choose the node isomorphic to the junction tree's first component.
% 
% \textbf{Overall Pipeline, Figure~\ref{fig:pipeline-detailed}.} The input is a set of molecules and their corresponding property values. 
% \tbd{1 sentence how to choose the meta G/DAG, and that this isn't critical}
% The goal is to learn an optimal latent geometry containing molecules both within and outside the training set, along with a graph diffusion model that predicts the property values of those molecules without property labels. 
%The latent geometry is derived from the grammar DAG, which consists of two parts: a stem DAG containing all possible tree structures precomputed by a small meta-grammar, and hanging leaves representing molecular graphs, each connected to one of those tree structures in the stem DAG.
% The stem DAG is constant and generalizable to different molecular datasets.
% Our approach learns how to attach molecules leaves to the stem DAG.
% We then learn a graph grammar as suggested in \cite{guo22}, but restrict it to contain only meta rules and molecular rules. %The latter determine how the molecules generated by the grammar are to be attached to the meta DAG. 
% Then, property prediction for new molecules is done by performing graph diffusion on the geometry graph.
% Thereby we jointly optimize the grammar (also molecular generator) and the property predictor.
%latent geometry.
% A joint optimization framework is proposed to optimize both the grammar DAG and the graph diffusion model.
% Note that we focus on a molecule generation scenario, where the goal is to predict properties for the molecules generated by the grammar. For property prediction over arbitrary molecules, the latter are given as additional input to the grammar learning.
% VT the below is maybe 
% In the following, we detail the hierarchical grammar, DAG construction, and joint optimization of grammar, also used as molecular generator, and property prediction. % our grammar DAG in detail in Sect \ref{sec:grammardag} and \ref{sec:hiergrammardag} and the bi-level optimization framework in Sect \ref{sec:graphdiff}.

\subsection{Hierarchical Molecular Grammars}\label{sec:hiergrammardag}

% mention here the size challenge
% VT commented for now, move somewhere... - maybe appendix
% Grammar DAG can provide all the possible graphs generated by a given grammar.
% In practice, however, constructing the grammar DAG is usually computationally intractable even for grammars with a limited number of production rules. 
% As a result of the combinatorial complexity of production rules, there are a large number of intermediate graphs. 
% This in turn dramatically increases the time required to perform isomorphism tests at each iteration of the BFS. 
% We test with random grammars learned from [] and find it is computationally impossible to construct the grammar DAG when there are more than ten production rules.
% \mh{TODO. State the difference of HMG from the previous MHG and the motivation}
% divide molecular generation into two stages 1 tree 2 specify molecular fragment, molecular rules follow previous paper
% Note that the meta rules have to be given in advance. but compact
% Since our initial experiments turned out that constructing a geometry as outlined above at runtime, based on an arbitrary, learned grammar \cite{guo22} is infeasible (for details see Appendix~\tbd{\ref{app:infeasible-dag}}), we propose to use a specific subset of grammars, carefully designed with feasibility in mind, by constraining the shape of the general grammars.

\textbf{Meta Grammars.} The formal definition of a meta grammar is as follows,
\begin{definition}\label{def:metagrammar}
%(\mathcal{N}, \Sigma, \mathcal{P}, \mathcal{X}
A \emph{meta grammar} $\metagrammar=(\mathcal{N}, \varnothing, \Pmc_{\metagrammar}, \mathcal{X})$ is a graph grammar, which only contains non-terminal nodes 
% $\mathcal{N}=\{\Rmcstar\}$ 
and only generates trees, i.e. $\forall w\in \{w|\Xmc\PGmetato w\}, w\in\mathcal{T}$. \\
% which generate trees over nonterminal nodes,
% A \emph{meta grammar} is a graph grammar which only contains meta rules. 
A meta grammar $\metagrammar$ is \emph{$k$-degree} if for all trees $T$ of maximal degree $\Delta(T) \leq k$, 
we have
%with $\deg(T)=\ell$ 
  $\Xmc\PGmetato T$.\\
A meta grammar~$\metagrammar$ % with rules $\Pmc$ 
is \emph{edit-complete} if for any tree pair $(T, T')$ with $|T|<|T'|$, tree edit distance $\ted(T,T')=1$, and $\Xmc\PGmetato T,T'$, 
there is a rule $p\in\Pmc_{\metagrammar}$ such that $T\pto T'$.\\ %, there is a rule $p\in\Pmc_\agrammar$ such that $T\pto T'$. 
% 
% new line because arrow subscript otherwise not readable
A k-degree, edit-complete meta grammar~$\metagrammar$ is \emph{minimal} if there is no other such %k-degree, edit complete 
meta grammar $\metagrammar'$ with~$|\Pmc_{\metagrammar'}|<|\Pmc_{\metagrammar}|$. 
% 1. $v_L, v_R \in \{\mathcal{R}^*\} \cup V_{anc}, \forall\ v_L \in V^{(i)}_L, v_R \in V^{(i)}_R$ \\
% 
\end{definition}%
% \textbf{Meta Grammar Construction.} 
% Discuss the definition, relation with junction tree.
% Discuss how to construct meta grammar
The three additional attributes %characterizations 
% \mh{I keep using the word ``charaterization'' to refer to the above three properties but I dont think it is quite accurate. Suggestions other than ``properties'' (since it conflicts with the molecular property) are welcomed!} 
in the above definition can be used to deduce nice characteristics of a meta grammar:
``Degree $k$'' ensures the meta grammar is expressive and complete, covering all possible trees under a simple tree degree constraint;
\mh{``Edit completeness'' allows explicit capture of transformations between two trees with one edit distance and therefore between two arbitrary trees;}
``Minimality'' 
% \mh{Not sure it should be ``minimum'' or ``minimality''} 
guarantees that the meta grammar is compact.
Based on these three attributes, we can construct a generic meta grammar generating trees of non-terminal nodes by using only a small but expressive set of production rules, which we refer to as \emph{meta rules}.
% helps with the construction of a small but expressive set of meta rules for our DAG. 
% However, since they only generate trees of nonterminals and are hence extremely generic, the construction of minimal meta grammars is straightforward. 
Figure~\ref{fig:motivation} shows a $3$-degree meta rule set and a derivation of a tree based on this rule set.
Each rule has one non-terminal node at $\mathit{LHS}$ and two non-terminal nodes at $\mathit{RHS}$.
% Consider the first rules in Figure~\ref{fig:motivation}: 
According to the number of anchor nodes at $\mathit{LHS}$, which is also the degree of $\mathit{LHS}$, $\{p_1\}$, $\{p_2\}$, $\{p_3, p_4\}$, and $\{p_5\}$ correspond to transformations of tree nodes with a degree from $0$ to $3$, respectively.
For each $\mathit{LHS}$ degree that is smaller than $3$, there is one rule whose $\mathit{RHS}$ maximal degree is increased by one by attaching a non-terminal node without changing the anchor nodes, i.e. $p_1$, $p_2$, and $p_4$.
The remaining transformations that satisfy the edit-complete constraint are captured by $p_3$ and $p_5$.
Minimality follows from the fact that there is no redundant rule in the rule set.
% to generate arbitrary trees, we only need one rule per degree, increasing the degree of a given nonterminal node by attaching a nonterminal node; to capture the remaining transformations (in a single step), we use \tbd{NUMBER} additional rules per degree that similarly attach a nonterminal node but also move some of the children of the given nonterminal.
It is evident that we can generate any possible tree with a degree smaller than $4$ by adopting a sequence of rules from this $3$-degree meta rule set.
More generally, to generate arbitrary trees with maximal degrees no greater than $k$, we construct meta grammars as follows, 
\begin{prop}
A meta grammar $\metagrammar$ with meta rules $\Pmc_{\metagrammar}$ constructed in Appendix~\ref{app:metarules} is of degree $k$, edit-complete, and minimal. 
% \mh{move to appendix, with proof}
\end{prop}
Appendix~\ref{app:metarules} provides the formulation of meta rule construction as well as proof that the three attributes are satisfied.
Generally speaking, we construct meta rule sets of arbitrary degrees by induction from $1$-degree meta grammar which consists of only one meta rule. 
In practice, a meta rule set with a reasonable degree should be chosen to ensure the coverage of most molecules.
% Observe that choosing meta rules with a reasonable degree ensures the coverage of most molecules we encounter in practice (for our experiment data, degree 4 was sufficient). 
In our experiments, we find it sufficient to use a meta rule set of degree $4$, which contains $8$ rules in total.
The simplicity of the meta rules shows that the main effort for constructing a hierarchical molecular grammar lies in the learning of the molecular grammar. 
% \textbf{Completeness.} 
% Lastly, we justify our grammar construction regarding the grammars from \cite{guo22}.
%The meta-rules are designed for generating only the internal framework of a molecule, while the molecular rules specify the framework with molecular fragments ($RHS$ of the rules).
% More specifically, we have following definition for \emph{k-degree} meta-rule set:
% Figure xxx shows an example of $3$-degree meta-rule set.
% \vat{stopped here}
% \begin{definition}
% A \emph{k-degree meta-rule set} is a production rule set $\mathcal{P} = \{p_i:H^{(i)}_{L}(V^{(i)}_L, E^{(i)}_L)\rightarrow H^{(i)}_{R}(V^{(i)}_R, E^{(i)}_R), i=1,..,n\}$ such that \\
% 1. $v_L, v_R \in \{\mathcal{R}^*\} \cup V_{anc}, \forall\ v_L \in V^{(i)}_L, v_R \in V^{(i)}_R$ \\
% 2. $H^{(i)}_{L}\overset{*}{\underset{\mathcal{P}}{\Rightarrow}}H^{(j)}_{R}$ iff $i=j$ \\
% 3. For any tree $T=(V_T, E_T)$ satisfying 1) $v=\mathcal{R}^*, \forall v\in V_T$; 2) its maximal degree $\Delta(T) \leq k$, there is a grammar derivation to $T$, i.e. $\mathcal{X}\overset{*}{\underset{\mathcal{P}}{\Rightarrow}}T$.
% \end{definition}
% The conditions ensure that a meta-rule contains only non-terminal nodes, that there are no redundant rules, and that the meta-rule set \vat{is expressive. ?; and also:
% In addition, the third condition facilitates the design of arbitrary $k$-degree meta-rule sets by using induction, as shown in the Appendix.}
% Note that the $k$-degree meta-rule set is extremely compact: with only $4$ rules, it is capable of generating all tree structures with degrees below $4$.
% In conjunction with molecular rules, the $k$-degree meta-rule set is capable of generating arbitrary molecules given by the following proposition,

\textbf{Hierarchical Molecular Grammars.} 
Based on meta grammar, we define hierarchical molecular grammar as follows,
\begin{prop}\label{prop:hmg}
A \emph{hierarchical molecular grammar} $\mathbf{G}=(\metagrammar, G_{mol})$ consisting of two graph grammars: 1) a $k$-degree, edit-complte, and minimal meta grammar $\metagrammar$ defined in Definition~\ref{def:metagrammar}; and
2) a \emph{molecular grammar} $G_{mol}=(\mathcal{N}, \Sigma, \Pmc_{mol}, \varnothing)$ where $\mathit{RHS}$ of any molecular rule in $\Pmc_{mol}$ only contains terminal nodes (i.e. atoms),
% whose RHS must not contain nonterminal nodes.\mh{Need more formal definition} %; they may generate arbitrary molecular fragments, that is, molecular graph structures over terminal nodes.
is a \emph{complete} grammar.
\end{prop}
``Completeness'' states that any molecular graph can be derived from a hierarchical molecular grammar with a set of appropriate molecular rules.
It can be demonstrated through the fact that every molecular graph can be decomposed into a tree-structured object (i.e. a junction tree using tree decomposition~\citep{diestel2005graph, jin2018junction}) whereas meta grammar is capable of generating trees of any degree. \mh{explanation on JT, motivation}
The role of molecular grammar is to transform a tree of non-terminal nodes produced by meta grammar into a molecular graph by specifying a molecular fragment for each non-terminal node.
Therefore, based on the molecular grammar, each molecule is associated with one tree generated by the meta grammar.
% Given that k-degree meta grammars are complete by definition - in that they are able to generate arbitrary trees - and that we have provided a constructive definition, it is left to mention that every molecule can be represented as a junction tree. The molecular rules are not restricted and thus can expand a nonterminal node to any molecular fragment.
% The molecular rules determine the relationship between molecules and trees, and thus affect the intrinsic geometry, so we choose to learn these rules.
In our approach, molecular rules are learned to optimize how molecules relate to trees and how grammar-induced intrinsic geometry is constructed.


\textbf{Molecular Grammar Learning.}\mh{explain more}
% \mh{Add rule construction formulation}
We follow the grammar learning from~\cite{guo2022data} but constrain the learned rules to molecular rules. 
Each molecule is considered as a hypergraph, and a set of hyperedges is sampled from the hypergraph iteratively until all hyperedges are visited. 
At each iteration, a molecular rule is constructed for each connected component.
% In order to construct molecular rules, a set of hyperedges is iteratively sampled in the hypergraph and a rule is constructed for each connected component until all hyperedges have been considered. 
An example is illustrated in Figure~\ref{fig:metagrammarJT}.
Following the hyperedge sampling process, a molecule can be converted into a junction tree.
We provide a detailed formulation of the constructed molecular rule and the resulting junction tree in Appendix~\ref{app:molrules}.
% The iterative sampling is achieved by defining a probability function $\phi(e,\theta)$ on each hyperedge $e$ with learnable parameters $\theta.
The iterative sampling follows i.i.d. Bernoulli distribution based on a probability function $\phi(e;\theta)$ defined on each hyperedge $e$ with learnable parameters $\theta$.
Hence, we convert the learning of molecular rules to the optimization of parameter $\theta$, which will be discussed in more detail in the following section.

% In a nutshell, a rule contains a nonterminal node together with the context of the selected edges on the LHS (i.e., anchor nodes describing the degree at the nonterminal), and the edges themselves together with the context on the RHS.
% Observe that, by design, our molecular rules learned model the construction of a junction tree.
% As outlined above, our construction is specific in that we constrain the learned rules to be molecular rules.
% the bottom-up grammar optimization methodology studied in [].
% Grammars are constructed by sampling hyperedges of molecular hypergraphs iteratively until all hyperedges have been visited.
% Our grammar construction differs from [] in terms of the form of the production rules, as our outputs are molecular rules.
% More specifically, consider the current graph $H_M = (V, E_H)$, we define a random variable
% Technically, \cite{guo22} define a random variable
% $X:\Omega\rightarrow\{0,1\}$ on each hyperedge~$e$, % $e\in E_H$. 
% which is sampled independently of other hyperedges and following a Bernoulli distribution, based on a probability function $\phi(e,\alpha)$ with parameters $\alpha$. 


% \subsection{Molecular Grammar DAG}\label{sec:grammardag}
% \mh{some of the content can be moved to preliminaries}
% A graph grammar can be used to generate graphs by sequentially applying production rules beginning with the starting symbol.
% Given a graph grammar $\mathscr{G}$, graphs are generated by sequentially applying production rules beginning with the starting symbol. 
% We can enumerate all possible graphs of $\mathscr{G}$ and construct a grammar DAG containing all these production sequences, denoted as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \tilde{\mathcal{H}})$.
% Each vertex of the DAG corresponds a \emph{unique} graph $\tilde{H}_i$, i.e. $\mathcal{V}=\{V_i| V_i \sim \tilde{H}_i, \mathcal{X}\overset{*}{\underset{\mathcal{P}}{\Rightarrow}}\tilde{H}_i, \tilde{H}_i\in \tilde{\mathcal{H}}\}$, where the root vertex corresponds the starting symbol $\mathcal{X}$ and each leaf vertex corresponds to a molecular graphs $H_i$.
% % where $\mathcal{V}=\{V_i|i=1,...,n\}$ is the set of intermediate graphs that are visited by BFS.
% Each edge is a directed edge and corresponds to a one-step grammar production $\mathcal{E}=\{(V_i, V_j)|\tilde{H}_i\underset{\mathcal{P}}{\Rightarrow}\tilde{H}_i, V_i\sim\tilde{H}_i, V_j\sim\tilde{H}_j, \tilde{H}_i, \tilde{H}_j\in \tilde{\mathcal{H}}\}$.
% Thus, each path from the root to a leaf represents the sequence of production steps to generate a certain molecule.
% To construct the grammar DAG, we perform breadth-first-search (BFS) from the starting symbol.
% \mh{could move following details to appendix}
% At each iteration of the BFS exploration, we enumerate all the production rules in the given grammar and test if each rule is applicable to the current DAG vertex. 
% When it occurs, we perform a one-step production on the current graph and check if there is any visited graph isomorphic with the produced graph. 
% Next, we either add a new child vertex corresponding to the produced graph to the current vertex, or add a directed edge from the current vertex to the visited isomorphic vertex. 
% The detailed algorithm is shown in Appendix.


\begin{figure*}[tb] %[]
\centerline{\includegraphics[width=0.8\linewidth]{.//figures/metagrammarJT.pdf}}
\vspace{-1.5ex}
% remember to say grammar DAG is a lower-dimensioanl representation than original graph representation. That is where intrinsic concept comes from
\caption{Overview of molecular grammar learning and grammar DAG construction. The rules of molecular grammar are constructed by iteratively sampling the hyperedges of the molecular hypergraph. Each molecule is then converted to a junction tree and attached to a node in the meta DAG corresponding to the isomorphic tree. \mh{legend. each colored node}}
\label{fig:metagrammarJT}
\vspace{-2.5ex}
\end{figure*}
\mh{Figure: how the meta DAG is constructed, from one black dot to another}


% \subsection{Property Prediction over Grammar-based Geometry}\label{sec:graphdiff}  

\subsection{Graph Diffusion over Grammar-induced Intrinsic Geometry}\label{sec:graphdiff}  

\textbf{Grammar-induced Intrinsic Geometry.}
% \textbf{Grammar DAG.}
% \mh{Use the Edit completeness to motivate the grammar-induced intrinsic geometry.}
As discussed in the previous section, any set of molecules can be generated by a hierarchical molecular grammar, each associated with one tree derived from the meta grammar. 
Therefore, we can measure the \emph{closeness} between two molecules using the tree edit distance between the trees they are associated with.
Based on the concept of closeness, a \emph{geometry} can be constructed where each molecule is represented as an element within this space, and the distance between these elements is calculated by using tree edit distances.
% Such a geometrical space captures the intrinsic structural similarity between molecules 
% Thanks to the edit completeness characterization of the meta grammar, this geometrical space can be explicitly constructed as the unit distance corresponds to a meta rule.
As compared to the \emph{embedding space} (or called \emph{latent feature space}) commonly used in machine learning algorithms, which uses the Euclidean distance to measure the closeness between elements~\citep{cayton2005algorithms}, the grammar-induced geometrical space is significantly different: Our geometry is  \emph{explicit and explainable}, where each unit distance along this space corresponds to a meta rule thanks to the edit completeness attribute of the meta grammar.
Since the tree edit distance used in the grammar-induced geometry reflects the structural similarity between molecular graphs, which is independent of any extrinsic molecular properties, we refer to this geometry as \emph{intrinsic geometry}.
We can explicitly construct the intrinsic geometry from a hierarchical molecular grammar by enumerating all production sequences in the grammar and represent all molecules that can be produced.

% \mh{Make all notations clear, states why using HMG for the DAG is more efficient}
Specifically, for a hierarchical molecular grammar, we build a grammar DAG where each node represents an intermediate graph resulting from a production sequence and each directed edge represents a production step between intermediate graphs.
As shown in Figure~\ref{fig:metagrammarJT}, the grammar DAG consists of two parts, a meta DAG which contains all the trees generated using meta rules, and molecular leaves which represent molecules and are attached to the trees in the meta DAG according to the molecular rules. \jc{Need to explain what a meta DAG means.}
The meta DAG is constructed by using breadth-first search originated from the starting 1-node tree $T_{start}=(\{\mathcal{X}\}, \varnothing)$. 
At each iteration, we enumerate all the meta rules that can be deployed to the tree represented by the current DAG node.
By using one-step production, we produce a new tree for each meta rule applicable.
A new child node representing the new tree is then created if it does not already exist in the current DAG, otherwise a directed edge is added between the current node and the matching existing node in the DAG.
For molecular leaves, since the hyperedge sampling process of molecular grammar learning provides the junction tree structure of molecules, each leaf is attached to the isomorphic tree in the meta DAG.
Appendix~\ref{app:grammardag} provides more details of the grammar DAG construction algorithm.
% \mh{Mention original MHG is not practical}
It is important to note that despite being of combinatorial complexity, the meta DAG construction, which contributes the majority of computation costs to the grammar DAG construction, is actually data-independent and can therefore be computed offline and applied across various molecular datasets.
Appendix~\ref{app:grammardag} includes an in-depth analysis of the computational cost reduction using our grammar DAG construction.

% In particular, we require it to explicitly capture the transformations between very similar graphs, and hence their closeness. 
% For a hierarchical molecular grammar, we construct a DAG as follows. The first part is based on only meta rules, data independent, and can be done offline. 
% (1)~Meta DAG: Given a set $\Pmc_{\mathit{meta}}$ of meta rules and the maximal node number $m$ for junction tree structures, we construct a DAG in which each node represents a tree derivable from the start symbol, the one-node tree $(\{ \Xmc\},\varnothing)$. Recall that each such tree  $T$ represents a set of molecules (i.e., junction trees), all those whose junction tree structure is isomorphic to $T$.
% We directly refer to the DAG nodes by their labels,
% and call a DAG node labeled by tree $T$ \emph{open} if 
% 1. $|V_T|< m$;
% 2. a rule $p$ can be applied to its tree, with $T \pto T'$;
% and 3. either (a) there is no DAG node labeled with $T'$, or (b) there is no edge between the nodes for $T$ and $T'$.
% Our DAG construction proceeds breadth-first as follows, until there are no open nodes in the DAG anymore: select an open DAG node as above and, if~(a) applies, extend the DAG by node $T'$ and edge $(T,T')$, otherwise add the edge $(T,T')$.
% We call this part of the DAG \emph{meta DAG}.
% (2)~Molecular DAG Leaves: At runtime, we extend $\Pmc_{\mathit{meta}}$ to a hierarchical molecular grammar by learning a set $\Pmc_{\mathit{mol}}$ of molecular rules; this part is similar to \cite{guo22} and detailed later. Correspondingly, we extend the meta DAG: for every node $T$ of its leaves, we add all possible molecules obtained by applying $\Pmc_{\mathit{mol}}$ to $T$ as successor nodes, such that each leaf represents a molecular junction tree.

% focusing on the given meta rules.
% Beginning with a root node for the start symbol \Xmc, representing hypergraph $H_0$, we model the applicable rules $p_i: H_0 H_{i,1}$ by connecting a fresh successor node labeled $H_{i,1}$
% by  
% Instead of considering a sequences
% Each  sequence of rule applications describes a directed acyclic graph
% \mh{Need to move the following paragraph to 4.2}
% For a hierarchical molecular grammar, the grammar DAG $\mathcal{G}_H$ is also decoupled into two parts: one is the DAG which is constructed using all the meta-rules, which we call \emph{meta-DAG}, denoted by $\mathcal{G}_{meta}$; the other is using molecular rules to derive molecules from those intermediate vertices in the meta DAG, denoted by $\mathcal{G}_H \setminus\mathcal{G}_{meta}$.
% It is possible to pre-compute and fix the meta DAG across different sets of molecules; only the molecular rules will need to be modified.
% Using this method, we are able to dramatically reduce the amount of time required to construct the whole grammar DAG for different molecule datasets.
% Note that our hierarchical molecular grammars focus entirely on representing junction trees in an efficient but expressive way; that is, they are technically grammars as proposed by \cite{guo22} but, while the latter learn arbitrary grammars based only on the given data, our meta rules are designed such that they can \emph{describe arbitrary data in an efficient way} and \emph{provide the right bias for property prediction learning}. The latter is particularly supported by designing the grammar such that it describes a DAG over trees, by considering extra rules capturing tree similarity (also demonstrated in our ablation study), and by using those as intrinsic geometry.
% \mh{A theoretical analysis on the efficiency and thus complexity reduction achieved is provided in Appendix~\ref{app:complexity-reduction}.} 

% Based on the grammar DAG, we define a geometry %$\mathcal{G} = (\mathcal{V}, \tilde{\mathcal{E}}, \tilde{\mathcal{H}})$ of 
% for molecules in form of a graph structure, by converting each directed edge of the DAG to an undirected one. Since the DAG is completely determined by the considered hierarchical molecular grammar, learning the geometry consists of learning the molecular rules of the grammar.
% Therefore, we first learn these rules and then build the grammar DAG, yielding the geometry and foundation for our property prediction using graph diffusion. The geometry and the diffusion model are optimized jointly. \mh{mention the graph distance gives the TED, insert and delete are invertible}

The intrinsic geometry is obtained by converting each directed edge of the grammar DAG to an undirected one, as shown in Figure~\ref{fig:diffusion}.
According to the grammar DAG construction, each node in this intrinsic geometry represents either a unique tree or a unique molecule. 
Each edge connecting two meta tree nodes corresponds to a meta rule and has a distance of 1 between its connected nodes due to the edit completeness of the meta grammar.
The distance between two arbitrary molecular leaves is the graph geodesic distance on the intrinsic geometry (i.e. the shortest-path distance).
Therefore, in this grammar-induced intrinsic geometry, molecules with similar underlying structures are closer, providing an informative prior for the learning of property prediction.

\textbf{Geometry-based Diffusion and Property Prediction.}
% \mh{Change title}\mh{DAG nodes for test and training}
As a widely used intrinsic operator on geometric data~\citep{crane2013geodesics, wang2019intrinsic}, graph diffusion is employed in our method to perform property prediction.
We apply graph diffusion over the grammar-induced intrinsic geometry as outlined in Figure~\ref{fig:diffusion}.
Following the GRAND graph diffusion model~\citep{chamberlain2021grand}, three learnable components are used in a graph diffusion process: an encoder function~$\varphi$ defined on all the nodes in the intrinsic geometry, a decoder function~$\psi$ defined on molecular leaves, and a graph diffusion process in Equation \ref{eq:diffusion}. %, parameterized by $\beta$. 
Specifically, the encoder~$\varphi$ yields the initial state of the diffusion process $\mathbf{U}_0 = \varphi(\mathbf{U}_\text{in})$, where $\mathbf{U}_\text{in}$ is the matrix form of the input features of all the nodes. % of the $d$-dimensional features for the diffusion process:
The decoder produces the predicted property values of all molecular leaves $\mathbf{u}_T = \psi(M\odot\mathbf{U}_T)$, where $\mathbf{U}_T$ is the node-feature matrix from the final diffusion state, $M$ is a binary mask that masks out the rows corresponding to non-molecule nodes, $\odot$ is the Hadamard product, and $\mathbf{u}_T$ is the resulting vector containing the property values for all molecular leaves.
Appendix \ref{app:implementation} provides more implementation details of the diffusion model.
% takes the feature of all the leaves in the latent geometry from the final diffusion state ($t=T$) and produces the property value.
% We found diffusion GNNs to be superior to other options \cite{hgcn?,others?} in our setting and therefore apply GRAND. % mention to show that we investigated in detail..

% We apply diffusion over the geometry graph~$\Gmc$ as outlined in Figure~\ref{fig:diffusion}. 
% Since GRAND \cite{bronstein22-grand} is generic in its three components, our approach can be considered as a framework that can similarly integrate latest technology.
% \tbd{As encoder input, we ...}
% Our encoder is defined on all $n$ vertices of the geometry graph and yields the initial state ($t=0$) of the $d$-dimensional features for the diffusion process: ${U}^{(i)}_0 = \varphi(\tilde{\mathcal{H}}_i)\in\mathbb{R}^{d}$, where $\tilde{\mathcal{H}}_i$ is the corresponding graph for vertex $V_i$ in the latent geometry.
% Our prediction focus is on the molecule nodes of $\Gmc$ (i.e., the leaves in the original grammar DAG), hence we apply the decoder to compute property values 
% %\begin{align}
%     $\mathbf{u}_T = \psi(M\odot\mathbf{U}_T)$
% %\end{align}
% for them, where $M\in\mathbb{R}^{n\times d}$ is a binary mask that masks out the rows corresponding to non-molecule vertices, $\odot$ is the Hadamard product, and $\mathbf{u}_T$ is the resulting vector containing the property values for all leaves.
% Our decoder takes the feature of all the leaves in the latent geometry from %the final diffusion state ($t=T$) and produces the property value.
% The graph diffusion follows the diffusion equation with the diffusivity matrix as the learning parameter.
% The diffusivity matrix $\mathbf{L}_\alpha$ is defined for each edge of $\mathcal{G}$, whose element is calculated by $L_{ij} = g(U_t^{(i)}, U_t^{(j)}; \alpha)$.
 

\begin{figure*}[tb]
\centerline{\includegraphics[width=0.75\linewidth]{.//figures/pipeline.pdf}}
\vspace{-1.5ex}
\caption{Grammar-induced geometry and graph neural diffusion. We obtain the grammar-induced geometry by converting each directed edge of the grammar DAG to an undirected one. Graph neural diffusion is employed over this geometry to perform property prediction.\mh{explain numbers}}
\label{fig:pipeline}
\label{fig:diffusion}
\vspace{-2.5ex}
\end{figure*}

% \textbf{Joint Optimization.}
% \mh{Change all bi-level opt}
Our optimization objective includes the learning of both the geometry and the diffusion model:
\begin{align*}
% &\min_{\alpha, (\varphi, \psi, \beta)}{l}(\mathbf{u}_T,  \hat{\mathbf{u}}) = \overbrace{\min_{\alpha}\underbrace{\min_{(\varphi, \psi, \beta)}{l}(\mathbf{u}_T,  \hat{\mathbf{u}})}_{\mathit{inner}}}^{\mathit{outer}},
&\min_{\theta, (\varphi, \psi, \alpha)}{l}(\mathbf{u}_T,  \hat{\mathbf{u}}) = \min_{\theta}\min_{(\varphi, \psi, \alpha)}{l}(\mathbf{u}_T,  \hat{\mathbf{u}}),
\end{align*}
where $\hat{\mathbf{u}}$ contains the ground-truth property values and $l(\cdot, \cdot)$ is a regression loss. 
Note that the intrinsic geometry is determined by the grammar DAG, which is only determined by the molecular rules, the molecular grammar learning parameters $\alpha$ are the only parameters relevant for obtaining the geometry. \jc{What is $\theta$?} \mh{Will refer content to Sect. 4.1}
Since $\theta$ and $(\varphi, \psi, \alpha)$ are two groups of independent variables, we exploit block coordinate descent~\citep{wright2015coordinate} to optimize the objective.
% The inner objective is totally differentiable with respect to the parameters, hence we can use gradient descent for optimization. For the non-differentiable grammar learning, which is due to the fact that the loss for learned grammars is based on the molecules generated with them, and the generation is not differentiable, we apply REINFORCE \cite{..} as suggested in \cite{guo22}.
% \mh{mention REINFORCE}
A detailed derivation is provided in Appendix~\ref{app:optimization}.
